Binarized Convolutional Neural Networks with Separable Filters for Efficient Hardware Acceleration

State-of-the-art convolutional neural networks are enormously costly in both compute and memory, demanding massively parallel GPUs for execution. Such networks strain the computational capabilities and energy available to embedded and mobile processing platforms, restricting their use in many important applications. In this paper, we push the boundaries of hardware-effective CNN design by proposing BCNN with Separable Filters (BCNNw/SF), which applies Singular Value Decomposition (SVD) on BCNN kernels to further reduce computational and storage complexity. To enable its implementation, we provide a closed form of the gradient over SVD to calculate the exact gradient with respect to every binarized weight in backward propagation. We verify BCNNw/SF on the MNIST, CIFAR-10, and SVHN datasets, and implement an accelerator for CIFAR-10 on FPGA hardware. Our BCNNw/SF accelerator realizes memory savings of 17% and execution time reduction of 31.3% compared to BCNN with only minor accuracy sacrifices.

==> sub/rebuttal.tex <==
%%% From the 1st reviewer $$$

\subsection{1.1 Weak Presentation}
\subsubsection{a. Unjustified and uncited claims}
%- Literature on neural nets exceeded 1.5 million publications (L70)
Using Google Scholar to search keyword "Neural Networks" can obtain $1,940,000$ results.
However, this is indeed an unjustified and uncited claim because we haven't inspect whether all of them are related with the neural networks in machine learning or other fields.
We will fix this claim with a better description for the prosperous of NN community.

\subsubsection{b. Confusing claims}
%- ..we leave the linear combination task to the two major reasons.. (L270)
The operation of convolution across different channels provides a summation of the feature maps from preceding layers, and the summation can be considered as a linear combination of the weights on the preceding layer.

%- optimize a feature map horizontally (L282)
%We agree L282 is not a good description of the trainable parameters, weights, $\gamma$'s and $\beta$'s.
What we would like to mention is that the two kinds of parameters $\gamma$'s and $\beta$'s introduced by batch normalization with scaling and shifting method will also help to optimize feature maps during gradient descent toward lower loss. 

%- statistic parameters (L276): appears to be a terminology problem
The statistic parameters are the mean and variance, which are dependent with the dataset.
If we stack a mini-batch of images/feature maps up, the statistic parameters are calculated vertically across the a image/feature map.

%- destructive pooling layer (L289): why is pooling operation so destructive?
We agree "destructive" is not a descriptive term for losing information.
We will change to "a pooling layer that losing information through sub-sampling."


\subsubsection{c. Vague statements}
%- a little bit on SVHN (L631): how much?
As listed in Tab.~\ref{tab:results} in our method $2$ outperforms method $1$ by $0.42\%$ on SVHN dataset.
We will add the amount of difference into this sentence. 

%- One thing interesting (L681): this entire sentence is vague. Cite the figure 5, avoid using the word "thing" etc.
In Fig.~\ref{fig:filter_draw} we can learn that the all-positive and all-negative filters are trained most frequently, and these two filters render the convolution to running sum calculation.  

%- Classification Accuracy (Error Rate) in caption of Table 2: These are two opposite measures. Which one is reported here?
The results are reported in terms of error rate.
We will clarify these confusing terms of the caption.

%- Method 1, Method 2, Method 3 in Section 5.2: Please use the terms that you came up with on Figure 4 here to make it easier for the reader to understand which methods you are referring to.
The two training method are defined with the titles of Sec.~\ref{sec:method_1} and Sec.~\ref{sec:method_2}.
However, it is still too vague to refer to the two methods without listing them formally in the context.
We will add a itemized list to clarify the name of our training methods.

\subsubsection{d. Citation style is non-conventional}
%- Max etal, Jose etal are the first names of the authors. The consensus is to use surnames or avoid using names but cite the paper wherever you mention it.
We will use the last names when citing previous works.

%- References list should contain all the co-authors, not only et.al. Moreover, please refer to the peer-reviewed and published versions of these articles (most of the arxiv citations are already published in peer reviewed conferences).
We will fix the reference with every authors' names, and update those new publication with conferences.

\subsubsection{e. Typos}
%- while the choice directly approximate -> while the choice 1 directly approximates (L256)
%- Therefore, We -> Therefore, we (L259 and a similar mistake in L582)
%- the dominate singular vectors -> dominant or largest (L308)
%- the there is no need to keep the real-valued filters -> remove "the" and "there is no need" is a part of speech phrase
We will fix all typos in the paper.

\subsection{1.2 Experimental Evaluation}
\subsubsection{Integrated VGG's results}

\begin{table}[]
\centering
\caption{Cifar10 Performance Comparison between Different Networks}
\label{my-label}
\begin{tabular}{|c|c|}
\hline
Dataset                                  & CIFAR10                       \\ \hline
\multicolumn{2}{|l|}{\textbf{VGG-like structure}}                        \\ \hline
Real-value Networks (VGG like structure) & 10.75\%                       \\ \hline
BniaryNet(Courbariaux et al., 2016)      & 11.40\%                       \\ \hline
BNNw/SFSVD                               & 14.12\%                       \\ \hline
\multicolumn{2}{|l|}{\textbf{AlexNet-like structrue}}                    \\ \hline
"AlexNet" in BCNN settings               & 10.58\%                       \\ \hline
"AlexNet" in BCNNw/SF Settings           & \multicolumn{1}{l|}{Training} \\ \hline
\multicolumn{2}{|l|}{\textbf{Other benchmark}}                           \\ \hline
Maxout Networks (Goodfellow et al.)      & 11.68\%                       \\ \hline
\end{tabular}
\end{table}

\subsubsection{Integrated original BNN's and CNN's results}

\subsection{1.3 Interpretability}
\subsubsection{(no explicit accuracy reported though on the very FPGA implementation)}
% Currently the paper only provides FPGA accelerator on CIFAR-10 showing 1.46X speedup, making it hard to tell the potential benefit for the method.
Please see Sec.~\ref{sec:fpga_analysis} for the details of FPGA analysis.

\subsubsection{Scalability}
%How does it scale up to simpler task/network as MNIST (included in the paper for Theano implementation) and more complex task/network (such as Alex-net)?
%please present results on at least one large-scale dataset, e.g. ILSVRC, with a larger network, e.g. Alex-net
\label{sec:scalability}
Scaling down is not an issue both in training and hardware implementation, which simply effects the input convolution layer due to the single channel image.
We explain the scaling up effects below:

BCNN with SF performs SVD on every filter, and we can perform SVD during either run-time or compiling-time.
Assuming SVD is a constant-time operation, if decomposing filters during run-time is adopted, the complexity is $O(E\sum_{i=1}^L (M_i M_{i-1})$, where $M_0$ is the number of channels of input images, $L$ is the number of convolutional layers, and $E$ is the number of epochs during training.
To avoid SVD during run-time, we can build a table beforehand in compiling-time, and building such a table for SVD results is a $O(2^{N^2})$ problem, where $N$ is the size of filters.

Considering the architecture of our network models, $M\approx 100 N$, if perform SVD during run-time, we must decomposing filters for more than $152.4$ million times while constructing a table require only $512$ SVDs.% for $3$-by-$3$ filter size and $33,5$ million SVDs for $5$ filter size. 
Therefore, we choose to implement networks with all $3$-by-$3$ filters because $3$-by-$3$ filters has been proven efficient in CIFAR-10, and the size of table is merely $512$, which is relatively easier for training.
However, if we scale the size of filters up, say $5$-by-$5$, the table size grows drastically to $33,554,432$ but still can be computed by a high-end GPU.
For larger filter sizes, perform SVD during run-time with a second order approximation to obtain the separable filters is suggested, which means a fast estimation of the mapping relationship between original binary filters and SVD results.

We have implemented a more complex network similar with Alex-Net and verified on CIFAR-10 again since the training on ILSVRC takes longer than one week.
The layer stack is is the same with those listed in Tab.~\ref{tab:archi}, but the number of kernels and filter sizes are different: 96x3x5x5 - 256x96x5x5 - 512x256x3x3 - 512x512x3x3 - 256x512x3x3 - 512x512x1x1.
The accuracy of the more complex network is $11\%$.

%%% From the 2nd reviewer %%%

\subsection{2. does not show very strong performance gain against BCNN}
% Not confident review
The goal of this paper is to modify neural networks to accommodate resource-limited hardware.
We trade in accuracy to shrink down the memory footprint and boost the speed in this work.

%%% From the 3rd reviewer $$$

\subsection{3.1 A low-level nature.}
%- The presentation style as well as the method itself are quite technical. Many of the steps have a low-level nature. The contribution is incremental.
The bottleneck of learning with separate filters is SVD, previous works cannot build a table of the SVD result because of real number filters has infinite possible combination.
Luckily, the binarized neural networks make the table building task computable if the size of filter size is small, see Sec.~\ref{sec:scalability} for some examples of filter sizes versus table sizes,

\subsubsection{3.2 The CV domain is not emphasized much}
%- The computer vision domain is not emphasized much. The method should be explained with a more explicit connection to it, similarly as it is done e.g. in [13].
Our work is very essential to computer vision domain because we further push the hardware accelerator for neural networks to a new limit.
As mentioned in Sec.~\ref{sec:intro}, although there exist many powerful network designs like AlexNet and GoogLeNet, the inference computation still relies too heavily on high-end GPU machine, and cannot be carried out to IoT or other mobile application cheaply.
Therefore, we aim at simple computer vision task recognizing small pattern and make binarized neural network more hardware-friendly in terms of the speedup and reduction of memory footprint.
This work accomplish the goal from the algorithm level down to a real hardware implementation.

\subsection{3.3 A more detailed analysis of the achieved results}
%- are the savings 17% and 31% model/data-independent? is it a significant improvement e.g. with respect to high-end IoT devices? how does it compare to savings achieved by other hardware-friendly models?
\label{sec:fpga_analysis}
The reduction in memory footprint and execution time is primarily due to the reduction in model size enabled by using separable filters to compress each 2D convolutional filter into two 1D vectors. The savings are data and device-independent and will be achieved as long as the network uses binary conv layers. The technique scales well to larger filters sizes since the memory is reduced by a factor of $2/n$. For comparison to other hardware-friendly models, this work specifically addresses binary neural networks, which may not be suitable for many optimizations. Separable filters can also complement many existing techniques such as input batching, tiling, and etc.



